Simulating Quantum Circuits by Model Counting

Quantum circuit compilation comprises many computationally hard reasoning tasks that nonetheless lie inside #$\mathbf{P}$ and its decision counterpart in $\mathbf{PP}$. The classical simulation of general quantum circuits is a core example. We show for the first time that a strong simulation of universal quantum circuits can be efficiently tackled through weighted model counting by providing a linear encoding of Clifford+T circuits. To achieve this, we exploit the stabilizer formalism by Knill, Gottesmann, and Aaronson and the fact that stabilizer states form a basis for density operators. With an open-source simulator implementation, we demonstrate empirically that model counting often outperforms state-of-the-art simulation techniques based on the ZX calculus and decision diagrams. Our work paves the way to apply the existing array of powerful classical reasoning tools to realize efficient quantum circuit compilation; one of the obstacles on the road towards quantum supremacy.

==> preamble.tex <==

\RequirePackage{color}

\RequirePackage{physics}
%\RequirePackage[utf8]{inputenc}
\RequirePackage{graphicx}
%\RequirePackage{epigraph}
\RequirePackage{amsmath}

%\RequirePackage[ruled,vlined]{algorithm2e}
\RequirePackage{algorithm}
\RequirePackage[noend]{algpseudocode}

\RequirePackage{amssymb}
\RequirePackage{braket}
%\RequirePackage{xfrac} %for sfrac

\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{thmtools}
\RequirePackage{xspace}
\RequirePackage{multirow}
\usepackage{colortbl}
\RequirePackage{stmaryrd}
\RequirePackage[colorlinks,citecolor=blue!60!black!70,linkcolor=blue!60!black!70]{hyperref}%\RequirePackage{cite}
\usepackage{appendix}
\RequirePackage{hyperref}
\RequirePackage{caption}
\RequirePackage{subcaption}
\RequirePackage{mathrsfs}
\RequirePackage[english]{babel}
% \RequirePackage{mathabx}
\RequirePackage{pgfplots}
\RequirePackage{calc}
\RequirePackage{nicefrac}
\RequirePackage{todonotes}
\RequirePackage{complexity}
%\RequirePackage{fdsymbol}
%\RequirePackage{eucal}
\RequirePackage{tikz}
\usetikzlibrary{shapes,backgrounds,calc,arrows,automata}
\usetikzlibrary{graphs,quotes}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{shapes,backgrounds,calc,arrows}
%\RequirePackage{verbatim}
\RequirePackage{soul}
\RequirePackage{wrapfig}
%\tikzstyle{every node} = [circle, draw,inner sep=3pt]
\let\clipbox\relax
\pgfplotsset{compat=1.18}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{empheq}
\usepackage{amssymb}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
\usepackage{hyperref}
\usepackage{qcircuit}
\usepackage{tabularx}
\usepackage{etoolbox}
\usepackage{arydshln}
\usepackage{mathtools}



\newcommand{\algstrut}[1][\algruledefaultfactor]{\vrule width 0pt
depth .25\baselineskip height #1\baselineskip\relax}


\newcommand*{\algrule}[1][\algorithmicindent]{\hspace*{.5em}\vrule\vrule
width 0pt height .75\baselineskip depth .25\baselineskip\hspace*{\dimexpr#1-.5em}}

\makeatletter
\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
    \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
    % do nothing
    \addvspace{-3pt}% FUDGE for cases where no text is shown, to make the rules line up
    \else
    \unskip
    % draw a rule for each indent level
    \ALG@printindent@tempcnta=1
    \loop
    \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
    \advance \ALG@printindent@tempcnta 1
    \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
    \repeat
    \fi
    \fi
}
\usepackage{etoolbox}
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{pifont}
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother

\AtBeginEnvironment{algorithmic}{\lineskip-2pt}


\newcommand*\Stateh{\State \algstrut[1]}


\interfootnotelinepenalty=10000

\RequirePackage[bottom,symbol]{footmisc} 
\RequirePackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$ {\footnotesize #1}}

\setlength{\parskip}{7pt}
\setlength{\parindent}{0pt}

\newcommand{\innerprod}[2]{\langle #1 | #2 \rangle}

\newcommand{\unit}{1\!\!1}
\def\X{X}
\def\Y{Y}
\def\Z{Z}
\newenvironment{algo}[1][Algorithm]
    {\begin{center} 
    \begin{tabular}{|p{0.9\textwidth}|} 
    \hline 
    \vspace{0.1\baselineskip} 
    \textbf{#1}\\} 
    { 
    \\\hline 
    \end{tabular} 
    \end{center} 
    \vspace{\baselineskip} 
    } 

% \newtheorem{example}{Example}

\newcommand{\diagonal}[1]{\begin{smallmat}1 & 0 \\ 0 & #1\end{smallmat}}
\newcommand{\antidiagonal}[1]{\begin{smallmat}0 & #1 \\ 1 & 0\end{smallmat}}

\makeatletter
% start with some helper code
% This is the vertical rule that is inserted
\renewcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%
\makeatother

\usepackage{caption}
\usepackage{MnSymbol}

\renewcommand\sectionautorefname{Section}
\renewcommand\subsectionautorefname{Section}
\renewcommand\subsubsectionautorefname{Section}
\renewcommand\figureautorefname{Figure}
\renewcommand\tableautorefname{Table}
\newcommand\exampleautorefname{Example}
\newcommand\algorithmautorefname{Algorithm}
\renewcommand\appendixautorefname{Appendix}
\newcommand*{\Appendixautorefname}{Appendix}
% \renewcommand\definitionautorefname{Definition}
\renewcommand\itemautorefname{Item}
% \renewcommand\lemmaautorefname{Lemma}
\renewcommand\theoremautorefname{Theorem}
\renewcommand\equationautorefname{Eq.}
\usepackage{bm}

